When Human Pose Estimation Meets Robustness: Adversarial Algorithms and Benchmarks

Human pose estimation is a fundamental yet challenging task in computer vision, which aims at localizing human anatomical keypoints. However, unlike human vision that is robust to various data corruptions such as blur and pixelation, current pose estimators are easily confused by these corruptions. This work comprehensively studies and addresses this problem by building rigorous robust benchmarks, termed COCO-C, MPII-C, and OCHuman-C, to evaluate the weaknesses of current advanced pose estimators, and a new algorithm termed AdvMix is proposed to improve their robustness in different corruptions. Our work has several unique benefits. (1) AdvMix is model-agnostic and capable in a wide-spectrum of pose estimation models. (2) AdvMix consists of adversarial augmentation and knowledge distillation. Adversarial augmentation contains two neural network modules that are trained jointly and competitively in an adversarial manner, where a generator network mixes different corrupted images to confuse a pose estimator, improving the robustness of the pose estimator by learning from harder samples. To compensate for the noise patterns by adversarial augmentation, knowledge distillation is applied to transfer clean pose structure knowledge to the target pose estimator. (3) Extensive experiments show that AdvMix significantly increases the robustness of pose estimations across a wide range of corruptions, while maintaining accuracy on clean data in various challenging benchmark datasets.

==> include/arxiv.tex <==

% all comparison results

\begin{table*}[h]
    \centering
    \caption{Comparison of different methods with HRNet-W32 backbone and input size as $256 \times 192$. All results are tested with ground truth bounding boxes.}
    \vspace{0.2cm}
    \scalebox{0.65}{
    \begin{tabular}{c|c|c|c|ccc|cccc|cccc|cccc}
\hline
Method & AP\_{clean} & mPC & rAP & Gauss.& Shot & Impulse & Defoucs & Glass & Motion & Zoom & Snow & Frost & Fog & Bright & Contrast & Elastic & Pixel & JPEG \\
\hline
Standard&
76.6&53.3&69.6&51.2&54.1&52.5&46.7&46.2&43.4&18.8&56.2&59.7&66.2&71.8&54.5&61.1&59.8&57.1\\
Standard$^*$&
74.4&53.0&71.3&51.3&54.2&52.6&46.9&46.3&43.5&19.2&55.9&59.1&65.2&70.3&54.1&60.5&59.4&56.9\\
+ FT&
77.0&53.3&69.2&50.8&53.7&52.0&47.0&46.3&43.7&18.6&56.7&60.2&66.6&72.2&54.9&61.4&59.0&56.4\\
+ FT$^*$&
75.0&53.1&70.9&51.1&54.1&52.3&47.2&46.4&43.8&18.9&56.5&59.5&65.8&70.9&54.6&60.8&59.0&56.4\\
Style&
75.2&56.2&74.8&55.3&58.2&57.6&49.0&48.7&46.6&19.4&61.1&61.3&67.2&71.5&60.3&61.4&64.7&60.7\\
+ Style&
76.1&54.8&72.0&50.5&53.0&53.4&49.3&47.8&46.6&21.6&59.4&59.8&66.9&71.4&57.2&61.6&63.5&60.0\\
+Style+AdvMix&
75.2&56.2&74.8&55.3&58.2&57.6&49.0&48.7&46.6&19.4&61.1&61.3&67.2&71.5&60.3&61.4&64.7&60.7\\
+Style+AdvMix+FT&
76.0&56.5&74.3&55.6&58.5&57.6&48.7&48.4&46.9&19.3&61.5&61.8&67.9&72.2&60.7&61.9&64.6&61.5\\
+Style+AdvMix+FT$^*$&
73.9&56.3&76.2&55.8&58.6&57.7&48.9&48.5&47.0&19.9&61.2&61.4&67.2&71.1&60.5&61.4&64.3&61.3
\\
\hline
    \end{tabular}}
    \label{method_comparison}
\end{table*}



% ablation study results

\begin{table*}[h]
    \centering
    \caption{Ablation study with HRNet-W32 backbone and input size as $256 \times 192$.}
    \vspace{0.2cm}
    \scalebox{0.7}{
    \begin{tabular}{c|c|c|c|ccc|cccc|cccc|cccc}
\hline
Method & AP\_{clean} & mPC & rAP & Gauss.& Shot & Impulse & Defoucs & Glass & Motion & Zoom & Snow & Frost & Fog & Bright & Contrast & Elastic & Pixel & JPEG \\
\hline
Standard&
76.6&53.3&69.6&51.2&54.1&52.5&46.7&46.2&43.4&18.8&56.2&59.7&66.2&71.8&54.5&61.1&59.8&57.1\\
+ Grid-Mask&
76.4&54.8&71.7&54.3&56.9&56.3&47.4&47.1&44.8&17.5&59.4&60.7&66.7&72.3&57.2&61.6&61.6&58.4\\
+ AutoAugment&
76.2&54.2&71.1&53.7&56.7&54.7&47.0&45.9&42.9&18.0&56.6&60.0&67.8&72.2&58.1&60.8&60.2&58.5\\
+ InstanceNorm&
76.4&53.8&70.5&52.7&55.4&53.8&46.5&46.2&44.0&17.1&58.3&60.0&66.3&72.0&56.6&61.2&60.4&57.0\\
Hierarchical&
76.2&54.6&71.6&54.1&56.9&55.6&47.0&46.4&44.1&17.4&58.9&60.5&66.8&72.3&58.0&61.0&61.2&58.4\\
Hierarchical + FT&
76.8&55.2&71.8&54.7&57.3&55.9&47.2&46.5&44.9&18.3&59.9&61.2&67.4&73.0&58.2&61.5&61.9&59.3\\
DirichletMix + FT&
76.9&55.5&72.1&55.4&57.9&56.3&47.2&46.5&44.5&17.5&60.4&61.5&67.8&73.3&59.4&61.7&62.1&60.4\\
RandomMix + FT&
76.9&55.3&71.9&54.9&57.6&55.8&47.1&46.4&44.5&17.7&60.1&61.4&67.6&73.2&59.3&61.6&62.3&60.2\\
AdvMix + FT&
76.7&56.1&73.1&56.0&59.1&57.8&48.3&48.0&45.2&18.0&61.1&62.4&67.8&73.0&59.2&61.8&62.8&60.6\\
\hline
    \end{tabular}}
    \label{benchmark}
\end{table*}

% +Joint Perturb&
% 76.4&53.8&70.4&52.5&55.3&53.6&46.8&46.3&44.1&17.2&58.3&60.0&66.3&71.9&56.7&61.0&60.3&56.6\\



% bottom up on COCO
\begin{table*}[h]
    \centering
    \caption{Benchmark of bottom-up human pose estimation models on COCO-C.}
    \vspace{0.2cm}
    \scalebox{0.6}{
    \begin{tabular}{c|c|c|c|c|c|ccc|cccc|cccc|cccc}
\hline
Method & Backbone & Input size & AP\_{clean} & mPC & rAP & Gauss.& Shot & Impulse & Defoucs & Glass & Motion & Zoom & Snow & Frost & Fog & Bright & Contrast & Elastic & Pixel & JPEG \\
\hline
\multirow{3}*{PifPaf}
& Resnet-50 & $641 \times 641$ &64.8&34.4&53.1&30.4&32.2&29.5&30.9&27.9&26.5&8.8&36.4&40.2&49.9&57.3&34.9&47.8&29.9&34.1\\
& Resnext-50 & $641 \times 641$ &64.1&32.4&50.6&28.0&29.6&26.9&27.6&23.9&23.9&7.6&35.5&39.0&48.9&56.5&33.3&46.1&27.5&32.5\\
& Resnet-101 & $641 \times 641$ & 68.3&40.6&59.5&38.0&39.4&36.6&36.9&34.6&31.6&11.2&42.6&46.6&56.0&62.0&42.4&52.6&37.2&41.3 \\
\hline
\multirow{3}*{HigherHRNet}
& \multirow{2}*{HRNet-W32}
& $512 \times 512$ & 67.1&39.9&59.4&34.2&37.0&35.2&35.1&32.5&34.0&12.5&43.3&47.6&54.9&60.6&43.4&50.3&42.2&35.0 \\
& & $640 \times 640$ &68.5&39.6&57.8&31.5&38.9&37.6&34.8&32.6&33.8&12.1&44.0&47.9&55.1&61.4&42.9&50.6&37.8&33.2\\
& HRNet-W48 & $640 \times 640$ &69.8&40.8&58.4&36.7&39.8&37.9&35.6&33.1&34.2&12.5&44.7&49.0&56.3&62.8&43.7&51.3&39.9&34.3\\
\hline
    \end{tabular}}
    \label{benchmark_bu_coco}
\end{table*}





% \begin{table}[h]
%     \centering
%     \caption{Comparison results on COCO-C of different methods with HRNet-W32 backbone and input size as $256 \times 192$. All results are tested with ground truth bounding boxes if not specially mentioned. FT means that we initialize our network by loading the existing well-trained weights. $*$ means results tested with detector having human AP of 56.4 on COCO val2017 dataset.}
%     \vspace{0.2cm}
%     \scalebox{1.0}{
%     \begin{tabular}{c|c|c|c}
% \hline
% Method & AP\_{clean} & mPC & rAP \\
% \hline
% Standard&
% 76.6&53.3&69.6\\
% +FT&
% \textbf{77.0}&53.3&69.2\\
% Standard$^*$&
% 74.4&53.0&71.3\\
% +FT$^*$&
% 75.0&53.1&70.9\\
% Style&
% 67.5&46.7&69.1\\
% +Style&
% 76.1&54.8&72.0\\
% +Style+AdvMix&
% 75.2&56.2& \textbf{74.8}\\
% +Style+AdvMix+FT&
% 76.0& \textbf{56.5}&74.3\\
% +Style+AdvMix+FT$^*$&
% 73.9&56.3&76.2
% \\
% \hline
%     \end{tabular}}
%     \label{method_comparison}
% \end{table}


% MPII-C & OCHuman


\begin{table*}[tb]
    \centering
    \caption{Benchmark of top-down human pose estimation models on MPII-C.}
    \vspace{0.2cm}
    \scalebox{0.65}{
    \begin{tabular}{c|c|c|a|a|ccc|cccc|cccc|cccc}
\hline
Backbone & Input size & AP\_{clean} & mPC & rAP & Gauss.& Shot & Impulse & Defoucs & Glass & Motion & Zoom & Snow & Frost & Fog & Bright & Contrast & Elastic & Pixel & JPEG \\
\hline
Resnet-50 & $256 \times 256$ & 88.5&77.5&87.6&68.9&71.6&68.9&84.2&85.3&83.6&53.7&70.0&75.6&83.1&86.6&69.1&87.8&87.8&86.8 \\
\hline
Resnet-101 & $256 \times 256$ & 
89.1&78.6&88.3&70.4&73.1&70.6&84.8&86.0&84.1&53.9&72.2&76.9&84.1&87.0&71.9&88.3&88.4&87.3\\
\hline
Resnet-152&$256 \times 256$ &
89.6&79.6&88.8&74.1&76.3&74.1&85.3&86.5&84.8&54.5&72.1&77.6&84.4&87.7&71.4&88.8&88.8&87.9\\
\hline
HRNet-W32& $256 \times 256$ & 90.3&80.1&88.7&71.5&74.1&72.4&86.0&87.0&85.3&56.0&73.8&78.6&86.1&88.5&74.5&89.5&89.5&88.7 \\
\hline
    \end{tabular}}
    \label{tab:benchmark_td_mpii}
\end{table*}




\begin{table*}[tb]
    \centering
    \caption{Benchmark of bottom-up human pose estimation models on OCHuman-C.}
    \vspace{0.2cm}
    \scalebox{0.6}{
    \begin{tabular}{c|c|c|c|a|a|ccc|cccc|cccc|cccc}
\hline
Method & Backbone & Input size & AP\_{clean} & mPC & rAP & Gauss.& Shot & Impulse & Defoucs & Glass & Motion & Zoom & Snow & Frost & Fog & Bright & Contrast & Elastic & Pixel & JPEG \\
\hline
\multirow{3}*{PifPaf}
& shufflenetv2x2 & $641 \times 641$ & 37.8&30.8&81.5&28.7&28.8&28.1&32.7&32.2&32.9&17.2&26.3&30.5&36.4&36.1&30.5&36.2&32.8&32.6\\
& Resnet-50 & $641 \times 641$ & 37.6&30.8&82.0&30.1&30.0&29.4&33.3&31.6&32.4&16.5&27.0&30.5&36.5&36.5&29.9&36.1&31.8&30.7\\
% & Resnext-50 & $641 \times 641$ & 36.3&27.7&76.3&27.0&27.3&26.7&28.6&26.0&29.3&14.2&24.5&27.4&34.6&34.2&26.6&33.5&28.8&26.7\\
& Resnet-101 & $641 \times 641$ & 39.6&34.9&88.1&35.6&35.6&35.3&37.2&35.3&36.3&20.2&31.4&34.4&39.2&38.8&34.8&38.9&35.5&34.6 \\
\hline
\multirow{4}*{HigherHRNet}
& \multirow{2}*{HRNet-W32}
& $512 \times 512$ & 40.0&35.1&87.6&32.9&33.1&33.2&37.3&36.5&36.9&21.7&31.6&36.0&39.9&39.4&36.9&39.2&37.1&34.4 \\
& & $640 \times 640$ & 39.3&33.6&85.4&30.9&31.1&31.8&36.2&35.0&36.1&19.6&31.1&35.1&39.3&38.1&35.8&38.3&33.8&31.1\\
& \multirow{2}*{HRNet-W48}
& $512 \times 512$ & 
41.7&36.7&87.9&35.5&35.6&35.7&38.8&37.5&38.5&22.0&33.5&37.6&41.5&40.5&39.0&40.6&38.0&35.6 \\
& & $640 \times 640$ & 40.9&35.4&86.4&33.0&33.3&33.5&37.7&36.6&37.6&21.1&32.4&37.4&41.5&39.9&37.2&39.9&36.6&32.6\\
\hline
    \end{tabular}}
    \label{tab:benchmark_bu_ochuman}
\end{table*}



==> include/intro.tex <==
\section{Introduction}

Human pose estimation (HPE) is a fundamental task for action recognition and video surveillance \cite{action_1, action_2, pose_surveilance}. Although convolutional neural networks (CNNs)  achieved great progress \cite{CPM, simple, hrnet, openpose, asso_embedding, higherhrnet} on challenging datasets \cite{coco, mpii, ochuman}, which only contain clean and high-resolution images, deploying models in the real world requires not only good performance on clean data, but also robustness to commonly occurring image corruptions. Unfortunately, unlike the human vision system, current pose estimators suffer severe performance drop when images are corrupted. Therefore, analyzing and enhancing the robustness of pose estimators are important and are the purposes of this work.


\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{figs/1st_page_v4.pdf}
\caption{\small \textbf{Comparisons} between HRNet without and with AdvMix, which significantly improves the standard HRNet in images with subtle JPEG compression (1st row) and Frost artifacts (2nd row). Please compare results of ground truth (left), HRNet (middle), and our HRNet+AdvMix (right).}
\label{fig:vis}
\end{figure}


Recent work on the robustness of CNNs can be categorized into adversarial robustness and corruption robustness. Firstly, adversarial robustness such as \cite{adv_robust_1, adv_robust_2, adv_robust_3, adv_robust_4, adv_robust_5, adv_benchmark_pose} mainly focuses on the robustness of neural networks towards worst-case adversarial examples, which are carefully designed by attackers. However, the samples generated by maximizing recognition errors (worst cases) may not naturally exist in real applications. 
%
Secondly, in contrast, corruption robustness pays attention to practical real-world image distortions such as noise, blur, and bad weather conditions. This work focuses on corruption robustness and tries to figure out how image quality affects the performance of pose estimators. 

Although there are recent studies on common robustness for classification, object detection, and semantic segmentation \cite{imagenet_benchmark, det_benchmark, seg_benchmark}, we are the first to conduct comprehensive evaluations for human pose estimation. Unlike classification, detection, and segmentation, HPE uses a blend of classification and regression methods to model the structures of the human body, making it a challenging and collaborative field that is worthy of special investigations.

Inspired by~\cite{imagenet_benchmark}, we evaluate advanced human pose estimators on a full spectrum of \textbf{unseen} corruption types, which are not encountered in model training (\ie CNNs are trained on \textit{clean} images, while evaluated on corrupted images). 
%
Our main contribution is to establish the robust pose benchmarks, consisting of three challenging datasets including COCO-C, MPII-C, and OCHuman-C. 
%
Extensive evaluations on these benchmarks show the \textbf{weaknesses} of both existing top-down and bottom-up pose estimators. (1) The state-of-the-art pose estimators suffer severe performance drop on corrupted images as shown in Fig.\ref{fig:vis} (\eg accuracy of HRNet-W32 with image size $256 \times 192 $ is reduced from 74.4 to 53.0 on COCO-C). (2) By comparing various types of image corruptions, we find that models are generally more robust to brightness and weather changes, while less robust to motion and zoom blur. (3) The model robustness would increase by increasing model capacity. %\jh{(4) We find that increasing the input resolution will harm the model robustness (\eg robust performance of ResNet-50 is 69.0\% vs. 66.1\% rPC for image size $128 \times 96$ and $384 \times 288$.).}


This work aims at improving robustness against different \textbf{unforeseen} corruptions. Extensive empirical evaluations on the proposed benchmarks help us screen a collection of useful data augmentation techniques to improve model robustness under severe corruptions. How can we make full use of these techniques and combine random augmented images to further improve the generalization of human pose estimators towards corruptions in our benchmark?
% However, we find that simply combining them sequentially does not achieve optimal performance. 
%
% As pointed out by \cite{generalization}, augmenting data from one specific corruption (\eg rotation) does not generalize well to another (\eg uniform noise).
%
To address this problem, we propose a novel data augmentation algorithm AdvMix, which \textit{learns} to automatically combine augmented images. Specifically, AdvMix jointly trains two neural networks in an adversarial manner, \ie an augmentation generator and a human pose estimator. The generator produces weights to mix up randomly augmented strategies, while the pose estimator attempts to learn robust visual representation from harder training samples. 
%
\jh{To reduce the effect of AdvMix-induced noise patterns}, we propose to use a pre-trained teacher pose estimator to transfer knowledge learned from \textbf{clean} training data in advance towards the target human pose estimator. 
%
Extensive evaluations demonstrate that AdvMix significantly improves model robustness on diverse image corruptions while maintaining performance on clean data.

%Data augmentation is a commonly used technique to improve the generalization of neural networks. However,  In this work, we aim at improving the general robustness against different unforeseen corruptions. Based on extensive empirical evaluations, we find a collection of useful augmentation techniques to improve the model robustness. However, we find that simply combining them sequentially does not achieve desirable performance. 

Our main \textbf{contributions} can be summarized as follows. 
\begin{itemize}
\item We propose three robust benchmarks COCO-C, MPII-C, and OCHuman-C, and demonstrate that both top-down and bottom-up pose estimators suffer severe performance drop on corrupted images, drawing the community's attention to this problem. This is also a critical problem to be addressed for deploying models in real applications. 

\item With extensive experiments, we have many interesting conclusions that would help improve the accuracy and robustness of future works.

\item We propose a novel adversarial data augmentation method together with knowledge distillation, termed AdvMix, which is model-agnostic and easy-to-implement. It significantly improves the robustness of pose estimation models while maintaining or slightly improving the performance on the clean data, without extra inference computational overhead.

\end{itemize}
